Scale-aware neural calibration for wide swath altimetry observations

Sea surface height (SSH) is a key geophysical parameter for monitoring and studying meso-scale surface ocean dynamics. For several decades, the mapping of SSH products at regional and global scales has relied on nadir satellite altimeters, which provide one-dimensional-only along-track satellite observations of the SSH. The Surface Water and Ocean Topography (SWOT) mission deploys a new sensor that acquires for the first time wide-swath two-dimensional observations of the SSH. This provides new means to observe the ocean at previously unresolved spatial scales. A critical challenge for the exploiting of SWOT data is the separation of the SSH from other signals present in the observations. In this paper, we propose a novel learning-based approach for this SWOT calibration problem. It benefits from calibrated nadir altimetry products and a scale-space decomposition adapted to SWOT swath geometry and the structure of the different processes in play. In a supervised setting, our method reaches the state-of-the-art residual error of ~1.4cm while proposing a correction on the entire spectral from 10km to 1000k

==> results.tex <==
\begin{tabular}{llrrrrrrrrr}
\toprule
{}            xp &       rmse &   grad\_rmse &   spat\_res\_mean &  spat\_res\_std &  \\
\midrule
     calibration model &     0.013922 &    0.006465 &          44.991787 &     14.161194 &         \\
     4DVarNet &       0.021685 &          0.009566 &                   68.703365 &          22.456666 \\
	UNet       &  0.023385 &   0.010735 &      80.192038 &     21.374617 \\
\bottomrule
\end{tabular}


==> results_ablation.tex <==
\begin{tabular}{llrrrrrrrrr}
\toprule
{}            xp &       rmse &   grad\_rmse &   spat\_res\_mean &  spat\_res\_std & \\
\midrule
     base &    0.013922 &    0.006465 &          44.991787 &     14.161194 &   \\
tgrs\_no\_decomp & 0.0216827 &   0.00958416 &  68.506 &  22.4284 \\
   no\_res &   0.021685 &    0.009566 &          68.684462 &     22.501356 &   \\
   no\_mix &   0.019368 &    0.009605 &          57.610785 &     16.674918 &   \\
   no\_xb &   0.170286 &    0.024656 &         121.735632 &     43.637274 &   \\
\bottomrule
\end{tabular}


==> results_decomp_sensitivity.tex <==
\begin{tabular}{llrrrrrrrrr}
\toprule
            xp &        rmse &   grad\_rmse &    spat\_res\_mean &  spat\_res\_std &   \\
\midrule
     base &   0.013922 &    0.006465 &         44.991787 &     14.161194 &       \\
     40x4 &   0.015434 &    0.006880 &         39.955086 &     14.299718 &       \\
     40x2 &   0.014354 &    0.006635 &         40.413823 &      8.413560 &       \\
     10x8 &   0.014785 &    0.006755 &         43.569394 &     12.476813 &       \\
     10x4 &   0.015593 &    0.006812 &         42.387847 &     10.511919 &       \\
     5x16 &   0.014119 &    0.006647 &         43.551781 &     13.133111 &       \\
      log &   0.014572 &    0.006469 &         41.590025 &     13.071608 &       \\
\bottomrule
\end{tabular}


==> results_gridded.tex <==
\begin{tabular}{llrrrrrrrrr}
\toprule
            xp &       rmse &   grad\_rmse &   spat\_res\_mean &  spat\_res\_std\\
\midrule
   sst\_xb &      0.014333 &     0.005994 &        37.229858 &     12.254236 \\
    xb\_oi &      0.021800 &     0.008405 &        42.509677 &     13.209170 \\
     base &       0.013922 &     0.006465 &        44.991787 &     14.161194 \\
\bottomrule
\end{tabular}

\begin{tabular}{llrrrrrrrrr}
\toprule
            xp &         rmse &   grad\_rmse &   spat\_res\_mean &  spat\_res\_std \\
\midrule
   4DVarNet-sst &        0.020471 &          0.008546 &                 47.235353 &          18.103727 \\
    DUACS-4nad &        0.0487905 &         0.0170251 &                140.13 &          43.48 \\
     4DVarNet-5nad &         0.021685 &          0.009566 &                 68.703365 &          22.456666 \\
\bottomrule
\end{tabular}


==> results_sizes.tex <==
\begin{tabular}{llrrrrrrrrr}
\toprule
            xp &        rmse &   grad\_rmse &   spat\_res\_mean &  spat\_res\_std & \\
\midrule
   base &   0.013922 &    0.006465 &        44.991787 &     14.161194 &     \\
  smaller &   0.014404 &    0.006222 &        42.421190 &      9.868140 &     \\
  bigger &   0.014855 &    0.007186 &        46.091154 &     14.361817 &     \\
   linear &   0.021284 &    0.010232 &        68.359143 &     20.979959 &     \\
\bottomrule
\end{tabular}


==> results_unet.tex <==
 \begin{tabular}{lrrrr}
\toprule
{} &      rmse &  grad\_rmse &  spat\_res\_mean &  spat\_res\_std \\
xp                   &           &            &                &               \\
\midrule
tgrs\_no\_decomp       &  0.023385 &   0.010735 &      80.192038 &     21.374617 \\
tgrs\_base            &  0.014559 &   0.006282 &      40.133856 &      9.596725 \\
tgrs\_no\_xb\_no\_decomp &  0.350050 &   0.059077 &     375.711468 &    258.177709 \\
\bottomrule
\end{tabular} 

